The Early Universe as a Probe of New Physics

The Standard Model of Particle Physics has been verified to unprecedented precision in the last few decades. However there are still phenomena in nature which cannot be explained, and as such new theories will be required. Since terrestrial experiments are limited in both the energy and precision that can be probed, new methods are required to search for signs of physics beyond the Standard Model. In this dissertation, I demonstrate how these theories can be probed by searching for remnants of their effects in the early Universe. In particular I focus on three possible extensions of the Standard Model: the addition of massive neutral particles as dark matter (through the use of several minimal models of dark matter), the addition of charged massive particles (through catalyzed Big Bang Nucleosynthesis), and the existence of higher dimensions (through its effects on BBN and galactic positron production). For each new model, I review the existing experimental bounds and the potential for discovering new physics in the next generation of experiments.

==> chapter1c.tex <==
\chapter{Charged Relics \label{Chapter:ChargedRelics}}

\par
In addition to dark matter, it is also possible that the early Universe contained a small abundance of exotic charged particles. 

\section{Experimental Constraints}

\par
{\bf Check the work in \cite{ Dimopoulos:1989hk,Kudo:2001ie,Byrne:2002ri,Perl:2001xi}}

\section{Catalyzed Big Bang Nucleosynthesis}

\par
Big Bang Nucleosynthesis (BBN) is the process by which the light nuclei in the Universe are formed, and is also a powerful tool for constraining new physics (for a review, see eg. Ref \cite{Sarkar}) . The theory relies on particle physics, nuclear physics, and general relativity to predict the abundances, and the results depend on a single parameter, the baryon-to-photon ratio, which can be measured from the cosmic microwave background \cite{Spergel:2003cb}. The predictions have proven accurate when compared to the observed abundances in older, metal-poor stars. Therefore the effects of new physics on nucleosynthesis also provide strong constraints on proposed models.

\par
For example, if there exist charged particles which survive to nucleosynthesis then they can affect the standard processes. The charged particles form bound states with light nuclei, which reduces the usual Coulomb repulsion of other nuclei, as well as changing the rates of the nuclear reactions. This results in a shift in the relative abundances of light nuclei \cite{Pospelov:2006sc,KT,KR}.

\par
This effect is most noticeable in the rarer elements such as Lithium-6 and Lithium-7. It was demonstrated in Ref \cite{Pospelov:2006sc} that the presence of charged relics with $\tau > 10^5 {\rm s}$ would produce additional \lisx\, primarily through the reaction 

\begin{displaymath}
(^4HeX^-)+ D \to ^6Li + X^- 
\end{displaymath}

\noindent
for which the cross section is approximately eight orders of magnitude larger than the primary channel in the Standard BBN,

\begin{displaymath}
^4He + D \to ^6Li + \gamma
\end{displaymath}

\noindent
In addition, in Ref \cite{Bird:2007} \we\ demonstrated that there is a region of parameter space which satisfies the constraints from \lisx\ production while also reducing the \lisv\ abundance. These results are reviewed in this section.

\par
The abundance of \lisv\ is one of the few problems with the standard BBN. Using the value for the baryon-to-photon ratio derived from the CMB anisotropy, which leads to consistent predictions for the other abundances of light elements, the relative abundance of \lisv is predicted to be $Y_{^7Li} \approx 4 \times 10^{-10} $. However observations of low metallicity stars gives a value of $Y_{^7Li} \approx 2-3 \times 10^{-10}$, which is a factor of a few smaller than predicted.

\par
There have been several proposed solutions for the \lisv\ problem. If the relevant nuclear reactions had been measured incorrectly, or if there were different rates in the early Universe, the predictions would be altered, however the possible corrections do not produce a significant change in the \lisv\ abundance   \cite{Coc:2003ce,Angulo:2005mi}. It is still a possibility that there is an unknown mechanism in which stars burn \lisv\ faster than current models predict \cite{StarBurn}, which would change the inferred primordial abundances. It is also possible that an unknown physical effect, or a new particle, in the early Universe could affect the BBN predictions. In Ref \cite{Jedamzik} it was demonstrated that a decaying relic with  $\tau \sim 1000-3000 {\rm s}$ could release enough energy to lower the \lisv\ abundances.

\subsection{Recombination of \bes\ and $X^-$}

\par
The most important aspect of the \lisv\ suppression via CBBN is the recombination of \bes\ with the charged relic, $X^-$. If the capture rate is too low, then the density of bound states will be too low for the catalyzed reactions to affect the primodial \lisv\ abundance.\
\par
The recombination rate also depends strongly on the properties of the bound state, \bex\ . 

\par
{\bf more detail needed here...}

\begin{equation}
< \sigma_{rec} v > = \frac{6 \times 10^3}{T_9^{1/2}} + \frac{1.9 \times 10^4}{T_9^{3/2}} exp(-1.40/T_9) + \frac{1.5 \times 10^4}{T_9^{3/2}} exp(-1.62/T_9)
\end{equation}

\noindent
where $T_9 \equiv T/10^9 {\rm Kelvin}$ is the temperature, and the rate is given in the standard BBN units of $N_A^{-1} cm^3 s^{-1} g^{-1}$. The first term corresponds to the non-resonant reactions

\begin{displaymath}
\begin{split}
&^7Be_{3/2} + X^- \to (^7Be_{3/2} X^-) + \gamma \to  (^7Be X^-) + k \gamma \\
&^7Be_{3/2} + X^- \to (^7Be_{1/2} X^-) + \gamma \to  (^7Be X^-) + k \gamma
\end{split}
\end{displaymath}


\noindent
while the other two terms correspond to resonances and captures to the excited states of \bes .

\par
It is also important that the bound states are not destroyed by thermal photons. The rate for this process is

\begin{equation}
<\sigma_{photo} > = (2.0 \times 10^8 + 3.0 \times 10^9 T_9^{-1} + 2.3 \times 10^{10} T_9^{-2} ) exp(-15.42/T_9)
\end{equation}

\noindent
The combination of the recombination rate and photodisintegration rates gives

\begin{equation}
-H T \frac{dY_{B}}{dT} = n_{B} Y_X(1-Y_B)<\sigma_{rec} v> - n_{\gamma} <\sigma_{photo}>
\end{equation}

\noindent
with the assumption that $n_X \gg n_B$.


\subsection{Catalyzed Reactions}

\par
Once the bound states of \bes\ have formed, there are several reactions which destroy the \bes\ nuclei and decrease the abundance of \lisv\ + \bes\. Some of these reactions are enhanced relative to the SBBN case, while other reactions are not possible in SBBN.

\par
The first reaction to be considered is the destruction of \bes\ by protons. The reaction

\begin{displaymath}
^7Be + p \to ^8B + \gamma
\end{displaymath}

\noindent
is significantly enhanced in the catalyzed form, $(^7BeX^-) + p \to ^8B + X^-$, but the threshold energy is too large for this reaction to occur at any significant rate. It is possible to catalyze this reaction as

\begin{displaymath}
(^7BeX^-) + p \to (^8BX^-) + \gamma
\end{displaymath}

\noindent
In this reaction, there is a reduction in the Gamov suppresion due to the Coulomb shielding of the \bes\ nucleus by $X^-$, as well as an increase in the rate due to the emitted photon having approximately five times more energy than in the non-catalyzed reaction. The non-catalyzed reaction has been well studied (see for example Ref. \cite{Baye:2000gi} for the properties of the S-factor), and is known to depend on the third power of the photon energy. Therefore, at first approximation the S-factor {\bf (explain S-factors here...)} is taken to be

\begin{equation}
S_{CBBN}(0) = S_{SBBN}(0) \left( \frac{\omega_{CBBN}}{\omega_{SBBN}} \right)^3 \frac{1}{0.37^2} \sim 15 \; {\rm keV \; bn}
\end{equation}

\noindent
where \we\ take $S_{SBBN}(0)=21 \; {\rm eV \; bn}$ and the factor of $1/0.37^2$ represents the effects of the mass and charge of $X^-$.

\noindent
This reaction also receives a significant contribution from the bound state resonances, with the most important being

\begin{displaymath}
(^7BeX^-) + p \to (^8X^-,n=2,l=1) \to (^8BX^-) + \gamma \quad \quad E_R = 167 \; keV
\end{displaymath}

\noindent
where the energy is given relative to the $(^7BeX^-) + p $ unbound system. The rate for this reaction is {\bf perhaps more detail here...}

\begin{equation}
<\sigma v> \simeq 1.6 \times 10^8 T_9^{-2/3} exp(-8.86/T_9^{1/3}) + 1.6 \times 10^6 T_9^{-3/2} exp(-1.94/T_9)
\end{equation}

\noindent
The non-resonant contribution is small relative to the resonant rate, and the bound states, $(^7BeX^-)$, are destroyed by p-burning until $T_9 \approx 0.2$.
\par
The bound states, $(^8BX^-)$, will $\beta$-decay into $(^8BeX^-)$ which remains stable for the lifetime of the charged relic. Once it decays, the remaining $^8Be$ decays into two $\alpha$-particles, but the amount of $^4He$ produced in this way does not alter the primordial abundance of Helium. It may also be possible for the reaction $(^8BeX^-) + n \to ^9Be + X^-$, resulting in a small abundance of primordial $^9Be$.

\par
The second reaction to be considered is destruction by neutrons. In the Standard BBN, the main  channel for \bes\ depletion is 

\begin{displaymath}
^7Be + n \to ^7Li + p
\end{displaymath}

\noindent
However as outlined in Ref \cite{}, this corresponding bound state reaction

\begin{displaymath}
(^7BeX^-) + n \to (^7LiX^-) + p
\end{displaymath}

\noindent
is not enhanced, as the widths of the $^8Be$ resonances which mediate the reaction are too large to be affected by the binding energies in any significant way.It has also been argued that the reaction 

\begin{displaymath}
(^7BeX^-) + n \to X^- + 2^4He
\end{displaymath}

\noindent
would be enhanced \cite{KT}, but this is not true. {\bf More detail here perhaps}

\par
From the relative magnitude of the proton and neutron destruction of \bes\ , as well as the relative abundances of protons and neutrons at the appropriate temperatures, it is clear the in CBBN p-burning is the dominate channel for suppressing the \bes\ + \lisv\ abundance.

\subsection{Internal Decays of $X^-$}

\par
Another possible destruction mechanism is through the decay of the charged relic in the bound state. The three main processes are:

\begin{list}{}
\item A: $(^7BeX^-) \to ^7Be + {\rm decay \; products} + {\rm hard} \; \gamma \to ^3He + ^4He + ...$ 
\item B: $(^7BeX^-) \to ^7Be(E \gg T) + {\rm background \; particles} + ... \to ^3He + ^4He + ... $
\item C: $(^7Be^*X^-) \to^3He + ^4He + ...$
\end{list}

\noindent
In the first case, the decaying $X^-$ produces a high energy photon which destroys the \bes\ nucleus. In this case, the decaying $X^-$ can release energies of $O(100 \; GeV)$ while the photodisintegration threshold for \bes\ is $E_{thr} \simeq 1.59 \; MeV$. In the second case, the decaying $X^-$ does not directly affect the nucleus, but instead release the \bes\ nucleus back into the background of thermal nuclei. Because the orbital energies of the \bes\ are of order $O(1\;MeV)$ in the bound state, the recoiling nucleus is sufficiently energetic as to be broken up by collisions with other nuclei and background particles. In the third case, the effect of being bound to a charged particle polarizes the \bes\ nucleus, effectively forming a superposition of the ground state with several excited states of the free nucleus. When the $X^-$ decays, this polarization is removed and the \bes\ excited states can decay into $^3He+^4He$.

\par
The efficiency of case A is calculated as follows. {\bf more detail here...}

\begin{equation}
P_{rad\;br} \simeq \int_0^{\infty} dr |\psi(r)|^2 \int_{E_{thr}}^{E_{max}} \sigma_{\gamma}(E) dn_{\gamma}(E)
\end{equation}

\noindent
Using the cross-section for $^7Be + \gamma \to ^3He + ^4He$, this gives

\begin{equation}
P_{rad\;br} \sim 10^{-4} \quad \quad E_{max} = 100 \; {\rm GeV}
\end{equation}

\noindent
which indicates that this mechanism is not sufficiently efficient, and does not constitute a significant channel for suppression of the \bes\ + \lisv\ abundance.

\par
In case B, the destruction rate depends on the relative rates of the slowing of the \bes\ nucleus and the reaction $^7Be +  p \to ^8B+\gamma$. \We\ estimate that an $O(MeV)$ nucleus will thermalize in $10^{-6} s$, while the rate for \bes\ destruction is significantly slower. Therefore this mechanism is also not significant. 

\par
In case C, the rate of destruction depends on the part of the bound state \bes\ wavefunction which corresponds to an excited nucleus. This can be approximated as

\begin{equation}
\sum |\frac{{\bf dE}_{0i}}{E_0 - E_i}|^2
\end{equation}

\noindent
{\bf is the numerator electric field?}where ${\bf dE_{0i}}$ is of order 1 MeV, and the energy difference is $(E_i - E_0) \geq 10 \; MeV $. From these typical values, it is clear that this mechanism is not efficient either, with less than $1 \%$ of recoiling nuclei decaying from excited states. 

\par
These three channels do not contribute significantly to the destruction of \bes\ nuclei, and therefore the effects of internal decays of the charged relic can be ignored.

\subsection{Internal Conversion Channels}

\par
Another possibility is that there is a second relic state, $X^0$, which has a similiar mass to $X^-$, and which can be a decay product of $X^- \to X^0 + {\rm charged \; particles}$. The most obvious choice is a weak-coupling, $X^- \to X^0 + W^-$, and in this case the $W^-$ boson can then hit the \bes\ nucleus in the bound state,$(^7BeX^-)$, and convert it into a \lisv\ nucleus,

\begin{displaymath}
(^7BeX^-) \to ^7Li + X^0
\end{displaymath}

\noindent
This reaction is shown in Figure \ref{Figure::LiBeConversion}. As the \lisv\ nucleus is more fragile, it is subsequently destroyed through the SBBN channels.

\begin{figure}
\psfig{file=Be-Li.eps,width=9cm,angle=0}
\caption{\label{Figure::LiBeConversion} The internal conversion of \bes\ to \lisv\ via a weak-boson exchange with $X^-$.}
\end{figure}

\par


\subsection{Abundance}

\par
The parameter space is given in Figure \ref{Figure:Li7abundance} along with the constraints from \lisx\ and \lisv\ abundances.

\begin{figure}
\psfig{file=BBN-X.eps,width=14cm,angle=0}
\caption{\label{Figure:Li7abundance} Combined constraints on the abundance and lifetime of charged relics. The gray region is excluded by overproduction of \lisx\, while the lines represent the region that can explain the observed \lisv\ suppression.}
\end{figure}

==> chapter1d.tex <==

\noindent {\bf ********} \newline
{\bf I am not sure if any of this section should be included...} \newline
{\bf ********} \newline

\par
The abundance of WIMPs can be calculated as follows. The Boltzmann equation that determines the evolution of the abundance is {\bf check that the notation on $n_{DM}$ is consistent}

\begin{equation}\label{EQ::DMB}
\frac{dn_{DM}}{dt} = <\sigma_{ann}v> n_{dm}^2 - 3 H n_{dm}
\end{equation}

\noindent
where the Hubble constant (during the radiation dominated era) is given by {\bf add some comments about entropy normalization}

\begin{equation}
H = g_*^{1/2} \frac{T^2}{M_{PL}} \left( \frac{\pi^2}{90} \right)^{1/2}
\end{equation}

\noindent
From Eq \ref{EQ::DMB}, it is apparent that the abundance 'freezes out' when $<\sigma_{ann} v > n_{DM} \approx H$. This gives the freeze out abundance as

\begin{equation}
n_{DM} = g_*^{1/2} \frac{T^2}{M_{PL} <\sigma_{ann} v>} \left( \frac{\pi^2}{90} \right)^{1/2}
\end{equation}

\noindent
which, when normalized with the entropy density $s = \sqrt{2 \pi^2/45} g_* T^3$ gives the yield

\begin{equation}
\frac{n_{DM}}{s} =  \frac{x_f}{g_*^{1/2}  M_{PL} m_{DM} <\sigma_{ann} v>} \left( \frac{\pi^2}{90} \right)^{1/2}
\end{equation}

\noindent
where $x_f \equiv m_{DM}/T$. As a fraction of the critical density, the dark matter abundance is {\bf check the numbers against Kolb-Turner since some are missing}

\begin{equation}
\Omega_{DM} h^2=  \frac{x_f s_0 h^2}{ 3 g_*^{1/2}  M_{PL}^3 H^2 <\sigma_{ann} v>} \left( \frac{\pi^2}{90} \right)^{1/2} = \frac{3.71\times10^{-11} GeV^{2} x_f}{ g_*^{1/2}   <\sigma_{ann} v>} 
\end{equation}

\noindent
Using the measured value of $\Omega_{DM} = 0.12$ gives the requirement of $<\sigma_{ann} v> \sim 10^{-9} GeV^{-2}$.

==> chapter1g.tex <==
%\subsection{Lee-Weinberg Limit}

%\par
%In addition to the abundance constraint, in which the model is required to reproduce the observed dark matter abundance, each model is also constrained by the requirement that the coupling constants are perturbative.Although there are no strict limits on when a parameter becomes non-perturbative, in this \thesis the limit will be set as $\kappa \lesssim  \sqrt{4 \pi}$ for each model.
%\par
% The result of this requirement is that in each model, there is a lower bound on the WIMP mass. For this reason, it has been traditionally assumed that WIMPs must be heavier than $ \sim 10 GeV$ \cite{Lee:1977ua,Vysotsky:1977pe}. 

%\par
%As an example, consider a generic fermionic WIMP. For fermions, the annihilation cross-section is of the form

%\begin{equation}
%\sigma_{ann} \sim \frac{1}{64 \pi} \left( \frac{ \lambda \; m_{DM}}{M^2} \right)^2
%\end{equation}

%\noindent
%where $m_{DM}$ is the WIMP mass and M is the mass of a mediator particle. Using Eq \ref{Eq::Abundance} and $\Omega_{DM} = 0.11$, the coupling constant must satisfy

%\begin{equation}
%\lambda > \frac{M^2}{m_{DM}} \sqrt{\sigma_{ann}} \approx 4\times %10^{-5} \frac{M^2}{m_{DM}}
%\end{equation}

%\noindent
%To avoid existing constraints on new forces below the electroweak scale requires $M \gtrsim O(100 \; GeV)$, and so requiring $\lambda$ to be perturbative requires $m_{DM} \gtrsim 10 \; GeV $.
% the couplings will become non-perturbative and therefore the usual calculation of the annihilation cross-section is invalid {\bf check the original Lee-Weinberg papers}. This is known as the {\it Lee-Weingberg window}. {\bf explain this better} For the purpose of this \thesis, it will be assumed that couplings are perturbative for $\kappa \lesssim \sqrt{4 \pi}$, although there is no precise division between perturbative and non-perturbative couplings.
, and is based on the belief that light WIMPs cannot annihilate efficiently. However several recent papers have demonstrated that it is possible to produce $O(GeV)$ mass WIMPs with the correct abundance using either scalar WIMPs \cite{Boehm:2003bt,Fayet:2004bw,Fayet:2004kz, Bird:2006jd}, or using certain models of fermionic WIMPs with enhancements to the effective couplings \cite{Bird:2006jd}. %In addition, most dedicated dark matter searches are insensitive to WIMPs with masses below a few GeV, with strong bounds on the scattering cross-sections limited to the range of $m_{DM} \gtrsim 10 \; GeV$. 


==> chapter2b.tex <==
\chapter{Extra Dimensions \label{Chapter:ExtraDimensions}}

\section{Overview}

\par
The possibility that there may exist hidden dimensions in our Universe has been considered for several centuries. The first serious research into such dimensions occured in 1915 with the four-dimensional general theory of relativity, and the five and six dimensional theories of Nordstrom \cite{Nordstrom}, Kaluza \cite{Kaluza}, and Klein \cite{Klein}. These theories were re-discovered in the 1970's with the realization that certain models of supersymmetry and superstring theory were only consistent in higher dimensional spacetimes.

\par
In 1998, the idea that the Universe could contain extra dimensions was revitalized with the realization that higher dimensions could solve several problems with Standard Model. It was realized that if the Standard Model fields were confined to a small region of the extra dimension \cite{Arkani-Hamed:1998rs}, or a three-dimensional membrane \cite{Randall:1999ee,Randall:1999vf}, while gravity acts in all dimensions, then gravitational forces could be made as strong as the other three forces without violating existing experimental bounds. In addition, these models allowed extra dimensions as large as $R \sim 1 \; mm$ which made it possible to search for extra dimensions in modern gravity experiments. Similiar models have also been used to explain the fermion hierarchy \cite{Arkani-Hamed:1999za,Huber:2000ie}, number of spacetime dimensions\cite{Chodos:1979vk}, dark matter \cite{Servant:2002aq,Cheng:2002ej,Cembranos:2003mr}, dark energy, inflation \cite{Levin:1994yw}, and non-singular alternatives to inflation \cite{Khoury:2001wf}.


\par
There are numerous models of extra dimensions. The main classes of models are

\begin{list}{}
\item {\it Universal Extra Dimensions (UED)} - The original models of extra dimensions introduced by Kaluza and Klein included no difference between the new dimensions and the usual dimensions of space, with the exception of compactification. In the UED model, all Standard Model fields are allowed to propagate through all dimensions. This also results in very strong constraints on the size of the extra dimensions. 
\item {\it Flat Braneworlds} - The second class of extra dimensional models involves 4D branes embedded in higher dimensional spacetimes. In these models, only gravity can propagate in all dimensions, while the Standard Model fields are restricted to the brane. Gravity experiments still require these extra dimensions to be compact.
\item {\it Warped Extra Dimensions} - In models with warped extra dimensions, the Standard Model fields are still trapped on a 4D brane. However the strong warping of the dimensions allows for large or even non-compact dimensions as the warping limits the range over which gravity can operate.
\end{list}

\noindent
In this section we will be considering constraints on the ADD model of flat extra dimensions with branes. However the methods used could also be applied to other models to provide additional constraints.

\section{Previous Constraints \& Searches}

\subsection{Collider Constraints}

\par
In the ADD model all particle process can emit gravitons, however due to the weak gravitation couplings the rates of graviton emmission are proportianal to inverse powers of the Planck energy $M_{PL}$. As such it is not possible to search for specific events.

\par
It is possible to search for missing energy due to the emission of large numbers of gravitons. At the Tevatron, searches have been conducted for the reaction $p \overline{p} \to {\rm jet} + \cancel{E}$ while LEP searched for the reactions $e^+e^ \to \gamma+\cancel{E}, Z^0 + \cancel{E}$. The combined results from LEP give the limits in Table \ref{Table:XDcollider} at $95\%$ c.l. \cite{PDG}

\begin{table}[h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
d & 2 & 3& 4 & 5 & 6 \\
\hline
$M_*$ & 1.60  TeV &1.20 TeV& 0.94 TeV& 0.77 TeV& 0.66 TeV \\ \hline 
R & 250 $\mu m$ & 3.2 nm & 0.012 nm & $4.5 \times 10^{-4}$ nm & $5.0 \times 10^{-5}$ nm \\ \hline
\end{tabular}
\end{center}
\caption{\label{Table:XDcollider} Lower bounds on $M_*$ and upper bounds on R, due to missing energy experiments at LEP. }
\end{table}


\subsection{Astrophysics Constraints}

\par
Extra dimensions can also be constrained by their effects in the Universe. In the early Universe, large numbers of Kaluza-Klein gravitons would have been created, which then decay to $\gamma$-rays which could be observed by several satellite based experiments. Using the measurements from EGRET and COMPTEL, an upper limit on the size of extra dimensions was calculated \cite{Hannestad:2001nq}, and the results are given in Table \ref{Table::ExtraDimensionBounds}. 

\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
& $d=2$ & $d=3$ &$d=4$&$d=5$& $d=6$ \\ \hline
 $M_*$ & 167 TeV & 21.7 TeV & 4.75 TeV & 1.55 TeV 
& $< 1$  TeV$$
\\ \hline
R& $0.022$ $\mu m$ & $2.5 \times 10^{-5}$ $\mu m$ &$1.1 \times 10^{-6}$ $\mu m$&$1.7 \times 10^{-7}$ $\mu m$& $>2.9 \times 10^{-8}$ $\mu m$ 
\\ \hline \hline
 $M_*$ & 3930  TeV & 146  TeV & 16.1 TeV 
& 3.4 TeV & 1 TeV \\
\hline R &$4.1 \times 10^{-5}$ $\mu m$ &$1.1 \times 10^{-6}$ $\mu m$&$1.7 \times 10^{-7}$ $\mu m$&$5.7 \times 10^{-8}$ $\mu m$&$2.9 \times 10^{-8}$ $\mu m$
\\ \hline
\end{tabular}
\caption{\label{Table::ExtraDimensionBounds} Bounds on the size of flat extra dimensions and the Planck mass from astrophysical experiments, with the first two lines representing bounds from neutron stars and the second two lines representing bounds from the $\gamma$-ray background {\bf check that these two are labelled right}. The size of the extra dimensions in given as an upper bound, while the Planck mass, related by $M_{*}^{d+2} = M_{PL}^2 R^d $}
\end{table}

\par
In addition to the KK gravitons in the early Universe, it is also expected that high energy astrophysical processes will produce Kaluza-Klein gravitons. In particular, neutron stars would produce a flux of KK gravitons which would then decay to photons. These high energy photons would both reheat the neutron star, and produce a $\gamma$-ray flux. These predicted effects have been used to provide further constraints on the size of the extra dimensions \cite{Hannestad:2001xi}, and the results are given in Table \ref{Table::ExtraDimensionBounds}.

\section{New Constraints}

\subsection{Nucleosynthesis Constraints}

\par
As demonstrated in our previous work \cite{Allahverdi:2003aq}, the presence of extra dimensions will also affect the relative abundance of the light nuclei. 

\par
In the standard cosmology, it is believed that in the early universe there was a period of rapid expansion known as inflation. This expansion is generated by the presence of a field, referred to as the {\it inflaton}, which then decays into the Standard Model fields and reheats the Universe. 

\par 
However if the Universe also contains extra dimensions, then some fraction of the energy released by inflaton decay will be in the form of Kaluza-Klein gravitons. Since the KK modes interact through gravity, they couple to the mass and energy of the inflaton, and as such are relatively insensitive to the precise details of the inflaton model. This also requires that every decay channel of the inflation, $\phi \to \psi_i \psi_j$, be paired with a KK-mode producing channel, $\phi \to \psi_i \psi_j + KK$.
\par
The KK modes produced in inflaton decays are expected to have lifetimes of several years, which results in their decay occuring after all light elements have been generated by Big Bang Nucleosynthesis. As a result of this delay in the release of some of the inflaton energy, the relative abundances of the light elements will be distorted compared to models without extra dimensions, and observed abundances can be then used to restrict the nature of the higher dimensions. 

\par
For the purpose of this calculation, it will be assumed that the inflaton decays primarily to Higgs bosons. The Feynman diagrams which contribute to this decay are given in Figure \ref{fig:3body}. As \we will demonstrate, the constraints on extra dimensions which result from this calculation depend on the energy released rather than the coupling constants. Therefore these constraints are relatively insensitive to which decays dominate. 

\begin{figure}[t]
\begin{center}
\epsfig{file=KKinfl.eps, width=14cm, angle=0}
\end{center}
\vskip .1in
\caption{\label{fig:3body} 
The Feynman diagram for emission of KK modes in the decay of the inflaton into a pair of the scalars $\psi$. }
\end{figure}

\par
Although there is a large range of masses and lifetimes for the KK-modes which are produced, any neutral relics which decay after recombination $(\tau_{KK} \gtrsim 10^{12} \;sec)$ will leave a signature in the $\gamma$-ray background, which provide a very strong bound \cite{Ellis:1990nb,Kribs:1996ac}. For neutral relics with shorter lifetimes, it is expected that constraints from the dissociation of light nuclei will provide a stronger bound \cite{Ellis:1990nb,Cyburt:2002uv}. From Ref. \cite{Cyburt:2002uv} the bound on the energy released by these decays is

\begin{equation}
\frac{\sum n_{KK} m_{KK}}{s \cdot } \approx 2\times 10^{-12} \; GeV
\end{equation}

\noindent
for $\tau_{KK} \gtrsim 10^{8} s$, while for $10^8 s > \tau_{KK} > 10^6 s$ the bound is

\begin{equation} \label{Eq:BBNbound}
\frac{\sum n_{KK} m_{KK}}{s \cdot } \approx 2\times 10^{-9} \; GeV
\end{equation}


\begin{figure}[t]
\begin{center}
%\raisebox{0ex}{\scalebox{0.7}{\mbox{\input{life11t.pstex_t}}}}
\epsfig{file=life11.eps, width=14cm, angle=0}
\end{center}
\caption{\label{fig:lifetimes} 
The lifetime of the KK gravitons as a function of mass is
indicated by the dashed line. The lifetime of the KK
radions is shown for $d=2$ (solid line) and for $d=6$ (dashed-dotted line). 
} 
\end{figure}

\noindent
For KK modes with lifetimes in this range, the masses are in the electroweak energy scale, and the decays are to Standard Model particles. The lifetime of the graviton modes is \cite{Han:1998sg}

\begin{equation}
\tau_{gr} \simeq 5 \times 10^{4} \;{\rm sec} \left( \frac{1 \; {\rm TeV}}{m_{KK}} \right)^3
\end{equation}

\noindent
while for the radions the lifetime is

\begin{equation}
\tau_{rad} \simeq 2(d+2) \times 10^{5} \; {\rm sec} \left( \frac{1\; {\rm TeV}}{m_{KK}}\right)^3
\end{equation}

\noindent
The precise lifetimes are plotted in Figure \ref{fig:lifetimes}.

\par
By using the requirement that $\tau \lesssim 10^8 \; sec$ for the KK mode to have a significant effect on BBN, a maximum mass can be calculated

\begin{equation}
m_{max}^{\rm gr} \simeq 80 {\rm GeV}; 
\qquad 
\begin{array}{l c c c c c c l }
m_{max}^{\rm rad}  & \simeq &  200, & 210, & 225, & 240, & 250 &
{\rm GeV},  
\\[.3ex] 
\text{for}\, ~ d & = & 2, & 3, & 4, & 5, & 6, & 
\end{array}
\label{mmax}
\end{equation}

\begin{figure}[t]
\begin{center}
\epsfig{file=logC.eps, width=15cm, angle=0}
\end{center}
\caption{\label{fig:LogC} 
The dependence of $C_{{\rm rad}}(x)$, as defined
in \eqref{decaykk}, on the ratio $x = m_{KK}^{\rm rad}/m_{\phi}$. Separate plots are given for the number of extra
dimensions $d= 3,4,$ and $6$. }
\end{figure}

\par
The density of KK modes is calculated by first calculating the ratio of emitted KK modes to inflatons. This ratio is parameterized as

\begin{equation}\label{decaykk}
\frac{n^i_{KK}}{n_{\phi}} = C_i(x) \frac{m_{\phi}^2}{M_{PL}^2} \quad \quad x = \frac{m^{i}_{KK}}{m_{\phi}} \quad \quad i = {\rm gr,rad}
\end{equation}

\noindent
{\bf show the calculation here}The functions $C_i(x)$ are plotted in Figure \ref{fig:LogC}. The entropy released by inflaton decay satisfies the relation

\begin{equation}
\frac{n_{\phi}}{s} \simeq \frac{3 T}{m_{\phi}}
\end{equation}

\noindent
which can be combined with the results of \eqref{decaykk} to give the energy density of the KK modes,

\begin{displaymath}
\sum_{KK}\frac{m^{i}_{KK} n_{KK}^{i}}{s} \simeq  3 B_i(x) \frac{3 T m_{\phi}}{M_*}  \left(  \frac{m^i_{max}}{M_*}\right)^{d+1}, \quad \quad x = \frac{m_{max}^i}{m_{\phi}}
\end{displaymath}

\begin{figure}[t]
\begin{center}
\epsfig{file=logB.eps, width=15cm, angle=0}
\end{center}
\caption{\label{fig:LogB} 
The dependence of $B_{{\rm rad}}(x)$ on the ratio $x = m_{max}^{\rm rad}/m_{\phi}$. Separate plots are given for the number of extra
dimensions $d= 3,4,$ and $6$. }
\end{figure}

\noindent
where $B_i(x) = \sum_{KK} m^i_{KK} C_i(m_{KK}^i/m_{\phi}) $. Since the KK mode masses are very close together, this sum can be replaced with an integral over $m_{KK}^i$,  

\begin{equation}
B_i(x) = \frac{S_d}{x^{d+1}} \int_0^x dy C_i(y) y^d 
\end{equation}

\noindent
where $S_d = 2 \pi^{d/2} /\Gamma(d/2)$ is the surface area of a d-dimensional sphere. The function $B_{rad}(x)$ is plotted in Figure \ref{fig:LogB}.

\begin{table}[p]
\begin{center}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|c||c|c|c|c|c|}
\hline 
$m_\phi$ & $d=2$ & $d=3$ &$d=4$&$d=5$& $d=6$
\\ \hline \hline
1 TeV & 35 TeV  & 13 TeV & 7.1 TeV & 4.5 TeV & 2.8 TeV
\\ 
2 TeV & 47 TeV  & 17 TeV & 9.1  TeV & 5.7 TeV & 3.4 TeV
\\
$M_*$ & 220 TeV  & 42 TeV &  15 TeV &
7.9 TeV &  4.0 TeV
\\ \hline
\end{tabular}
\caption{\label{Table::EDBBN1} Lower bounds on the Planck mass from nucleosynthesis constraints.}
\end{center}
\end{table}


\begin{table}[p]
\begin{center}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|c||c|c|c|c|c|}
\hline 
$m_\phi$ & $d=2$ & $d=3$ &$d=4$&$d=5$& $d=6$
\\ \hline \hline
1 TeV & $0.52 \mu m$  & $6.0 \times 10^{-5}\mu m$ & $5.9 \times 10^{-7}\mu m$ & $3.9 \times 10^{-8}\mu m$ & $7.4 \times 10^{-9}\mu m$
\\ 
2 TeV & $0.29 \mu m$  & $3.8 \times 10^{-5}\mu m$ & $4.1 \times 10^{-7}\mu m$& $2.8 \times 10^{-8}\mu m$ & $5.7 \times 10^{-9}\mu m$
\\
$M_*$ & $0.013 \mu m$ & $8.5 \times 10^{-6}\mu m$ &  $1.9 \times 10^{-7}\mu m$ &
$1.8 \times 10^{-8}\mu m$ &  $4.6 \times 10^{-9}\mu m$
\\ \hline
\end{tabular}
\caption{\label{Table::EDBBN2} Upper bounds on the size of flat extra dimensions from nucleosynthesis constraints.}
\end{center}
\end{table}

\par
In the limit of $m_{max} << m_{\phi}$, the energy density of KK modes can be approximated as

\begin{equation}
\frac{\sum_{KK} m_{KK}^i n_{KK}^i}{s} \simeq \frac{2 S_d}{(d+1)\pi} \frac{T_R m_{\phi}}{M_*} \left[ \frac{d}{d+2} \left( \frac{m_{max}^{rad}}{M_*} \right)^{d+1} + 2 \left(\frac{m_{max}^{gr}}{M_*} \right)^{d+1} \right] \ln \left( \frac{m_{\phi}}{m_{max}} \right)
\end{equation}

\noindent
where \we take $\ln m^{gr}_{max} \approx \ln m^{rad}_{max}$, and $T_R \simeq 0.7 \; MeV$ is the reheat temperature. The constraint in Eq \ref{Eq:BBNbound} then places a constraint on $M_*$, and therefore on the scale of the extra dimensions. These limits are given in Table \ref{Table::EDBBN1} and Table \ref{Table::EDBBN2}.

\subsection{Galactic Positron Constraints}

\par
In the previous section \we considered the effects of Kaluza-Klein excitations in the early Universe. However it is also possible that quasi-stable modes, which still exist in the Universe, could provide an effect in the present.

\par
In this section \we consider the possibility that a significant density of KK gravitons could get trapped in the gravitational potential of the galaxy, leading to a halo surrounding our galaxy. Although these modes are quasi-stable, some will decay into electron-positron pairs and into $\gamma$-rays, which should result in an observable flux of $\gamma$-rays from direct decay and from electron-positron annihilation. The observed flux can then be used to constrain the nature of the extra dimensions \footnote{During the preparation of this thesis, \we\ became aware of another paper addressing this issue \cite{KK511}. However in that paper, only a single moduli field was considered rather than the complete spectrum of KK-modes}.

\par
As outlined in Section \ref{Section::LDM}, measurements by the SPI spectrometer on the INTEGRAL satellite \cite{Jean:2003ci} have confirmed previous observations of a flux of $511 \; {\rm keV}$ photons from the galactic center \cite{oldflux}. These experiments have also determined that these $\gamma$-rays are produced by a diffuse source rather than by a few point sources, which is consistent with a galactic halo composed of KK-modes. 

\par
The decay width and abundance of gravitons are given in \cite{hlz} and
 \cite{Hall:1999mk,Macesanu:2004gf} respectively. 

\begin{equation}\label{Eq:KKabundance}
\Omega_{KK} = (3.2 \times 10^{-3}) \frac{S_{n-1}}{\rho_{cr}} \frac{M_P T_0^3}{M_*^{d+2}} \int_0^{\infty} d m_{KK} \; m_{KK}^{d+1} \; \left(  \int_{m_{KK}/T_*}^{\infty} dx \; x^3 K_1(x)  \right) {\bf Check this equation, }
\end{equation}

\par
For the purpose of this calculation, it is assumed that the galactic halo is composed of the same distribution of KK-modes as given for cosmic scales in Eq \ref{Eq:KKabundance} and that this distribution is uniform with distance from the galactic center. It is possible that the constraints could be relaxed with a more realistic distribution of modes.

\begin{table}
\label{Table::PosBound}
\begin{displaymath}
\begin{array}{|c|c|c|c|c|c|}
\hline
d&  2 &3 &4 & 5 & 6 \\
\hline
R & & & & & \\ 
\hline M_* &&&&&  \\ \hline
\end{array} \end{displaymath}
\caption{Bounds on the extra dimensions from galactic positrons}
\end{table}

\par
The bounds on the size of the extra dimensions are given in Table \ref{Table::PosBound}.

==> chapter3c.tex <==
\subsection{Galactic Positron Constraints \label{Section:PosEX}}

\par
In the previous sections,the effects of Kaluza-Klein excitations on the early Universe were considered. However it is also possible that observable effects could be created in the modern Universe by quasi-stable modes, which the ADD model predicts would still exist in the present. 

\par
As outlined in Section \ref{Section::LDM}, measurements by the SPI spectrometer on the INTEGRAL satellite \cite{Jean:2003ci} have confirmed previous observations of a flux of $511 \; {\rm keV}$ photons from the galactic center \cite{oldflux1,oldflux2,oldflux3}. These experiments have also determined that the $\gamma$-rays are most likely produced by a diffuse source rather than by a few point sources, which is consistent with a galactic halo composed of dark matter or KK-modes. 

\par
In this section I consider the possibility that a significant density of KK gravitons could be trapped in the gravitational potential of the galaxy. %, forming a component of the dark matter halo. 
Although these modes are quasi-stable, some will decay

%\footnote{In addition to the decay of relic particles, positrons can also be produced in the annihilation of particles. However in this model the KK-mode annihilation cross-section is suppressed by a factor of $M_{PL}^2$ relative to the KK-mode decay width, and is not expected to provide an observable signal.} 

into electron-positron pairs and into $\gamma$-rays. This should result in an observable flux of $\gamma$-rays both from direct decay of the KK-modes and from subsequent electron-positron annihilation. The observed flux can then be used to constrain the nature of the extra dimensions by comparing the predicted flux with the observed flux in the solar system.
\footnote{During the preparation of this dissertation, \we\ became aware of another paper addressing this issue \cite{Kasuya:2006kj}. However in that paper, only a single modulus field was considered rather than the complete spectrum of KK-modes}.
\par
It should be noted also that the constraint considered in this section is a result of the production of low-energy positrons which lose energy as they travel through the interstellar medium. It is assumed that the positrons become non-relativistic within a short distance and annihilate in the galactic bulge. However the energy loss by these positrons and the cut-off energy at which the positrons can no longer contribute to the observed flux are not well understood, and cause some uncertainty in the final limits. For this reason, I will give the bounds for several energy cut-offs.
\par
It is also possible to detect relativistic positrons produced by dark matter annihilations or KK-mode decays in astrophysics experiments \cite{Baltz:1998xv,Hooper:2004bq,Hooper:2004yc}, with some experiments indicating an unexplained excess of high energy positrons \cite{Barwick:1997ig}. However there are also a number of uncertainties inherent to modelling positrons flux through the galaxy (see eg. Ref .\cite{Delahaye:2007fr}), and as such these bounds will not be considered in this \thesis.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\par
For the purpose of this calculation, it can be assumed that the $\gamma$-ray flux which results from KK decay depends only on the partial decay width and galactic abundance of the modes. It will also be assumed that all low-energy positrons produced in the decay of KK-modes will become non-relativistic and will contribute to the observed $511 \; keV$ flux.
\par
The decay widths for graviton decay to electron-positron pairs % or to $\gamma$-rays are 
is given in Ref. \cite{Han:1998sg}, 

\begin{equation}
\Gamma_{e^+e^-} (m_{KK}) \approx \frac{m_{KK}^3}{80 M_{PL}^2} 
\end{equation}

\noindent
while the abundance of gravitons in the Universe was previously calculated in Ref. \cite{Hall:1999mk} and Ref. \cite{Macesanu:2004gf}. At cosmic scales, the density of KK-modes as a function of mass is

\begin{equation}\label{Eq:KKabundance}
\Omega_{KK}(m_{KK}) = (3.2 \times 10^{-3}){\rho_{cr}} \frac{M_{PL} T_0^3}{M_*^{d+2}}  m_{KK} \; \left(  \int_{m_{KK}/T_*}^{\infty} dx \; x^3 K_1(x)  \right) 
\end{equation}


\noindent
where $m_{KK}$ is the mass of the Kaluza-Klein mode, $\rho_{cr}$ is the critical density of the Universe, $T_0$ is the temperature of the Universe, and $M_*$ is the reduced Planck mass. %It is assumed that the distribution of KK-modes is the same in the galactic halo as at cosmic scales, and that this distribution is not dependent on the distance from the galactic center. 

\par
From the cosmological KK-mode abundance, %given in Eq \ref{Eq:KKabundance} , 
the number density of KK modes in the galaxy and their spatial distribution can be approximated by 

\begin{equation}
n_{KK}(r,m_{KK}) = \frac{\Omega_{KK}(m_{KK})}{\Omega_{DM}}  \frac{\rho_{DM}(r)}{m_{KK}}
\end{equation}

\noindent
where $\Omega_{DM}$ is the total cosmic dark matter abundance, and

\begin{equation}
\rho_{DM} (r) = \rho_0 exp \left( -\frac{2}{\alpha} \left[ \left(\frac{r}{r_0} \right)^{\alpha} - 1 \right] \right)
\end{equation}

\noindent
with $r_0 = 20h^{-1} kpc$ and $0.1 < \alpha < 0.2$,is the galactic dark matter distribution \cite{Navarro:2003ew}. The constant $\rho_0$ is determined by requiring $\rho_{DM} (8.5 kpc) = 0.3 \; GeV/cm^3$, which is the accepted value of the dark matter density at the Solar system. In this calculation it is assumed that the KK modes are evenly distributed in the halo, and with the same mass distribution as in the early Universe. In practice the lightest modes are too light to be captured in the halo, however the effect of these missing modes is small. 

\par
Using this approximation for the density and distribution of Kaluza-Klein gravitons in the galaxy, the $\gamma$-ray flux can be determined using the decay width and branching ratio for the decays $KK \to e^+e^-$. Denoting the KK-mode decay width by $\Gamma_{KK}$, and the branching ratio to electron positron pairs by $BR_{e^-e^-}$, the number density of non-relativistic positrons produced per unit time is

\begin{equation} \label{Eq:PosDen}
N_{511 keV} (r) = S_{d-1} \int_0^{m_{max}} d m_{KK} \; m_{KK}^{d} 2 n_{KK}(r) \Gamma_{KK} BR_{e^-e^+}
\end{equation}

\noindent
As outlined in Ref \cite{Picciotto:2004rp}, the resulting flux of $511 \; keV$ $\gamma$-rays at the Solar system can be derived by calculating the line-of-sight integral of this density. 

\par
As discussed in the introduction to this section, the $511 \; keV$ flux has been measured by several experiments. The SPI spectrometer on the INTEGRAL $\gamma$-ray observatory measured
 an azimuthally symmetric distribution of $511\; keV$ photons with FWHM
 of $~9^\circ$, with an uncertainty covering the range 
$6^{\circ} - 18^{\circ}$, and total flux $\Phi_{obs} = 9.9^{+4.7}_{-2.1} \times 10^{-4} \; ph \; cm^{-2} \; s^{-1}$ \cite{Jean:2003ci}. Integrating the density in Eq \ref{Eq:PosDen} over
 this solid angle with the line of sight integral gives a total predicted flux of

\begin{equation}
\begin{split}
\Phi_{th}&= S_{d-1} \int_0^{m_{max}} d m_{KK} \; m_{KK}^{d-1}\frac{\rho_0 ( BR_{e^+e^-})}{2 \pi \tau_{KK}} \frac{\Omega_{\phi}}{\Omega_{DM}}  \int d\theta \int_{los}  \; exp \left( - \frac{2}{\alpha} \left[ \left( \frac{r}{r_0} \right)^{\alpha} -1 \right] \right)   ds \\&\\
&= S_{d-1} \int_0^{m_{max}} d m_{KK} \; m_{KK}^{d-1} \frac{BR_{e^+e^-}}{ \tau_{KK}} \frac{\Omega_{KK}}{\Omega_{DM}} (8.84_{\alpha=0.1} - 4.70_{\alpha=0.2})\times 10^{44}  \; cm^{-2} \; s^{-1}
\end{split}
\end{equation}

\noindent
Comparing this result with the observed $511 \;keV$ $\gamma$-ray flux constrains the mass and partial width of the particle,

\begin{equation}\label{DMC}
S_{d-1} \int_0^{m_{max}} d m_{KK} \; m_{KK}^{d+1} \frac{ \tau_{KK}}{BR_{e^+e^-}}\frac{\Omega_{DM}}{\Omega_{KK}}   \geq  (8.94_{\alpha=0.1} - 4.74_{\alpha=0.2})\times 10^{47} 
\end{equation}

\noindent
where it is assumed that the contribution from direct production of $511 \; keV$ photons is negligible. Although it is possible to produce a flux of $\gamma$-rays in this energy range through direct production, the effect is expected to be small and will not significantly alter the constraints given.


\par
Using these formulae and the decay width of the KK-gravitons, the constraint on $M_*$ can be written as,

\begin{equation}
\frac{d+4}{S_d} \frac{M_*^{d+2}}{m_{max}^{d+4}} \geq (5.92_{\alpha=0.1} - 3.16_{\alpha=0.2})\times 10^{33} GeV^{-2}
\end{equation}

\noindent
where as before $S_d = 2 \pi^{d/2} / \Gamma(d/2)$ and $m_{max}$ is the maximum KK mode mass which produces non-relativistic positrons. The corresponding bounds on the Planck mass and the size of the extra dimensions are given in Table \ref{Table::PosBound} and Table \ref{Table:PosBound2} respectively, for three choices for the upper bound on the KK-mode mass, and in Figure \ref{Figure:PositronBound} and Figure \ref{Figure:PositronBound2} for the range of $10 \;MeV < m_{max} < 1 \; GeV$. 

\begin{table}

\begin{center}
\begin{tabular}{|c|ccccc|}
\hline &d=2&d=3&d=4&d=5&d=6\\ \hline 
$m_{max} = 100 \; MeV$ &&&&&\\ \hline
$\alpha=0.1$ & 8870 & 254 & 22.9 & 4.03 & 1.08\\ 
$\alpha=0.2$ & 7580 & 224 & 20.7 & 3.69 & 1.00\\ \hline
$m_{max} = 50 \; MeV$ &&&&&\\ \hline
$\alpha=0.1$ & 3140 & 96.3 & 9.10 & 1.65 & 0.45\\ 
$\alpha=0.2$ & 2680 & 85.0 & 8.20 & 1.51 & 0.42\\ \hline
$m_{max} = 10  \; MeV$ &&&&&\\ \hline
$\alpha=0.1$ & 280 & 10.1 &  1.07 & 0.21 & 0.061\\ 
$\alpha=0.2$ & 240 & 8.93 & 0.96 & 0.19 & 0.056\\ \hline 
\end{tabular}
\caption{\label{Table::PosBound}Limits of sensitivity on $M_*$ (TeV) for different values of $\alpha$ and different dimensions. In addition, three different values of the maximum mass at which non-relativistic positrons are produced are given. }
\end{center}
\end{table}


\begin{table}
\begin{center}
\begin{tabular}{|c|ccccc|}
\hline &d=2&d=3&d=4&d=5&d=6\\ \hline 
$m_{max} = 100 \; MeV$ &&&&&\\ \hline
$\alpha=0.1$ & 8.0 pm & 0.42 pm &
    0.10 pm & 0.045 pm & 0.027 pm\\ 
$\alpha=0.2$ & 11.0 pm & 0.52 pm &
    0.12 pm & 0.051 pm & 0.029 pm \\ \hline
$m_{max} = 50 \; MeV$ &&&&&\\ \hline
$\alpha=0.1$ & 64.2 pm & 2.1 pm & 
    0.41 pm & 0.16 pm & 
    0.084 pm\\ 
$\alpha=0.2$ & 88.0 pm & 2.6 pm & 
    0.48 pm & 0.18 pm & 
    0.094 pm \\ \hline
$m_{max} = 10  \; MeV$ &&&&&\\ \hline
$\alpha=0.1$ & 8.0 nm & 91.0 pm & 
    10.2 pm & 2.84 pm  &
    1.2 pm\\ 
$\alpha=0.2$ & 11 nm & 112 pm & 
    12.0 pm & 3.2 pm & 
    1.4 pm \\ \hline 
\end{tabular}
\caption{\label{Table:PosBound2} Limits of sensitivity on the size of extra dimensions, R  for different values of $\alpha$ and different dimensions. In addition, three different values of the maximum mass at which non-relativistic positrons are produced are given. }
\end{center}
\end{table}

\par
It should be noted that these bounds are based on several assumptions. First, there is an assumption that the relative abundance of KK modes of different masses is the same in the galaxy as in the early Universe. Although heavier modes decay faster than lighter modes , as indicated in Figure \ref{fig:lifetimes}, the lifetimes are sufficiently long and the masses sufficiently small that this should not affect the distribution. There are also uncertainties in the dark matter halo profile of the galaxy, which can affect the observed flux, although this variation is small for most reasonable profiles and parameters. It is also assumed that the positrons annihilate within a short distance compared to the scale of the galactic center. This diffusion process is not completely understood, and if the positrons travel further then the observed flux would have a wider angular distribution which could improve these bounds \cite{Beacom:2004pe}. It is also assumed that all annihilating positrons produce $511 \; keV$ photons. However if a significant fraction of the positrons annihilate at higher energies, these photons would not be counted in the observed $511 \; keV$ flux. This would result in less stringent constraints on the number of positrons, and would weaken the bounds given in Table \ref{Table::PosBound} and Table \ref{Table:PosBound2}.
\par
There is also some uncertainty in the mass cut-off used. In this \thesis, a range of maximum masses was given with the assumption that heavier KK-modes will not produce nonrelativistic positrons. However the positrons produced in these decays will lose energy as they travel through the interstellar medium, and can become non-relativistic outside of the galactic bulge. It is also possible for heavier KK-modes to decay to $e^+e^-\gamma$ where the photon carries a large energy, resulting in additional low energy positrons. These two effects will increase the observable flux and would strengthen the constraints given in this \thesis.

\begin{figure}
\begin{center}
\psfig{file=pos-bound.pdf,width=\textwidth,angle=0}
\end{center}
\caption{\label{Figure:PositronBound} Bounds on $M_*$ as a function of the maximum Kaluza-Klein mode mass which produces non-relativistic positrons. }
\end{figure}

\begin{figure}
\begin{center}
\psfig{file=positron-bound2.pdf,width=\textwidth,angle=0}
\end{center}
\caption{\label{Figure:PositronBound2} Bounds on R as a function of the maximum Kaluza-Klein mode mass which produces non-relativistic positrons. }
\end{figure}

\par
From Table \ref{Table::PosBound}, it is apparent that the accumulated KK modes in the galactic core provide a strong bound on the size of the extra dimensions in the ADD model. It is also expected that other models of extra dimensions can be constrained in this manner as well. The bounds depend on the maximum mass of KK mode which is trapped in the galaxy. If KK modes heavier than $\sim 50 \; MeV$ can exist in the galaxy with a significant abundance and can produce nonrelativistic positrons, then the bounds from galactic positron production are stronger than the bounds from the extragalactic $\gamma$-ray background and other astrophysics experiments, as presented in Table \ref{Table::ExtraDimensionBounds}. 

\par
However it should also be noted that production of nonrelativistic positrons requres $m_{max} \lesssim O(100 \; MeV)$ \cite{Boehm:2003bt}, while limits on $\gamma$-ray production by bremsstrahlung processes suggest \footnote{It should be noted that these bounds assume all positrons are created with uniform energy. In this model, the positrons have a range of energies and so the upper limit on the Kaluza Klein mode mass can be higher than this without violating these bounds.} $m_{max} \lesssim 40 \; MeV$ \cite{Beacom:2004pe} or $m_{max} \lesssim 6 \; MeV$ \cite{Beacom:2005qv}. If these bounds are used as a mass cut-off, the resulting bounds are weaker than from other astrophysics constraints on the ADD model.

\par
In summary, Kaluza-Klein gravitons which were produced in the early Universe can still exist in the present. Furthermore, these particles can accumulate in the galactic halo, leading to a high density in the galactic core. When these modes do decay, they inject photons and positrons into the galaxy which could be observed by existing experiments. As an example, I derived the non-relativistic positron density in the galaxy which is produced by the decay of light KK-modes. By requiring the flux of such particles to be lower than the observed fluxes, such as was done with the $511 \; keV$ $\gamma$-ray flux in this section, strong limits can be placed on the properties of extra dimensions.

